Visually Grounded Speech Models have a Mutual Exclusivity Bias

When children learn new words, they employ constraints such as the mutual exclusivity (ME) bias: a novel word is mapped to a novel object rather than a familiar one. This bias has been studied computationally, but only in models that use discrete word representations as input, ignoring the high variability of spoken words. We investigate the ME bias in the context of visually grounded speech models that learn from natural images and continuous speech audio. Concretely, we train a model on familiar words and test its ME bias by asking it to select between a novel and a familiar object when queried with a novel word. To simulate prior acoustic and visual knowledge, we experiment with several initialisation strategies using pretrained speech and vision networks. Our findings reveal the ME bias across the different initialisation approaches, with a stronger bias in models with more prior (in particular, visual) knowledge. Additional tests confirm the robustness of our results, even when different loss functions are considered.

==> data_setup.tex <==
\section{Data setup}
\label{sec:data_setup}

We need a multimodal dataset containing isolated spoken words paired up with natural images for training, or images containing isolated natural objects for development and testing.
To do this, we combine multiple image and speech datasets to get one large dataset.  
For the image side, we use MSCOCO~\cite{lin_microsoft_2014} and Caltech-101~\cite{fei-fei_one-shot_2006} since there are object segmentations available for these datasets.
MSCOCO contains 328k images of 91 objects in their natural environment, and Caltech-101 contains Google images from 101 classes in the Webster Collegiate Dictionary.
To get the test and development image samples, we use the available ground truth segmentations to segment out the object corresponding to either a familiar or novel class.
The training images are natural images and not isolated objects.
All images are resized to 224$\times$224 pixels and normalised with means and variances calculated on ImageNet~\cite{deng_imagenet_2009}.

To get audio samples, we use the Flickr8k Audio captions corpus~\cite{harwath_deep_2015}, the Buckeye corpus~\cite{pitt_mark_a._buckeye_2005} and the LibriLight corpus~\cite{kahn_libri-light_2020}.
The Flickr8k Audio corpus contains five parallel spoken English captions for each image of the 8k images.
We only use the audio utterances (not the images).
The Buckeye corpus of English conversational speech are from 40 speakers, whereas the Libri-light set are 60K hours of audio from the LibriVox project.
We use forced alignments to segment out spoken words from the familiar and novel classes. 
Where forced alignments were not available for the audio datasets, we use the Montreal forced aligner~\cite{mcauliffe_montreal_2017} to generate alignments.
All words are parametrised as mel-spectograms with a hop length of 10~ms, a window of 25~ms and 40~mel bins. 
These are truncated or zero-padded to 256 frames.

\begin{table}[tb]
	\caption{Five examples of familiar and novel classes.}
	\label{tab:classes}
	\centering
	\scriptsize
	\setlength{\tabcolsep}{0.25em}
	\renewcommand{\arraystretch}{1.2}
	\begin{tabular}{ cc }
		\toprule
		Familiar & Novel \\
		\midrule
		dog & piano\\
		horse & camera\\
		umbrella & guitar\\
		boat & trumpet\\
		elephant & ball\\
		\bottomrule
	\end{tabular}
\end{table}

We divide this large multimodal dataset we put together into 13 familiar classes and 20 novel classes where five examples from each set are shown in Table~\ref{tab:classes}.
Next, we will briefly set out the class selection process.

\noindent\textbf{Step 1:} We manually evaluate which classes of Caltech and MSCOCO are viable.
I.e. which classes can be segmented out and still be legible. 
For example, the class \textit{curtains} are exluded since you cannot tell from the segmented out images that curtains are depicted.

\noindent\textbf{Step 2:} We make sure there aren't any conflicting classes. 
Examples of conflicting classes are dog and dalmation, and pigeon and bird. 
Therefore, images from ‘subclasses’ like dalmation and husky are added to the dog class.

\noindent\textbf{Step 3:} For the familiar set of classes, we check that there are more than 100 audio and image samples. 
If there are not, we rather add the classes to the novel set given that there are enough samples for testing.

Concretely, we use the spoken words paired with the entire natural images from the 13 familiar classes to train the model. 
During testing, we then use the spoken words paired with isolated natural objects from the 20 novel classes and the 13 familiar classes, to do the mutual exclusivity task described in Section~\ref{sec:me_task}.


==> defined_acronyms.tex <==
\DeclareAcronym{davenet}{
	short = DAVEnet ,
	long  = deep audio-visual embedding network,
	alt = Deep Audio-Visual Embedding Network
}
\DeclareAcronym{resdavenet}{
	short = ResDAVEnet,
	long  = residual deep audio-visual embedding network,
	alt = Residual Deep Audio-Visual Embedding network
}
\DeclareAcronym{AE}{
	short = AE ,
	long  = autoencoder
}
\DeclareAcronym{CAE}{
	short = CAE,
	long  = correspondence autoencoder,
	alt = Correspondence Autoencoder
}
\DeclareAcronym{MCAE}{
	short = MCAE,
	long  = multimodal correspondence autoencoder,
	alt = Multimodal Correspondence Autoencoder
}
\DeclareAcronym{MTriplet}{
	short = MTriplet,
	long  = multimodal triplet network,
	alt = Multimodal Triplet Network
}
\DeclareAcronym{FFNN}{
	short = FFNN,
	long  = feedforward neural network,
	alt = Feedforward Neural Networks
}
\DeclareAcronym{CNN}{
	short = CNN,
	long  = convolutional neural network,
	alt = Convolutional Neural Networks
}
\DeclareAcronym{RNN}{
	short = RNN,
	long  = recurrent neural network,
	alt = Recurrent Neural Networks
}
\DeclareAcronym{VQ}{
	short = VQ,
	long  = vector-quantisation
}
\DeclareAcronym{mfcc}{
	short = MFCC,
	long  = mel-frequency cepstral coefficient
}
\DeclareAcronym{CPC}{
	short = CPC,
	long  = contrastive predictive coding,
	alt = Contrastive Predictive Coding
}
\DeclareAcronym{multdavenet}{
	short = MultDAVEnet,
	long  = multilingual deep audio-visual embedding network,
	alt = Multilingual Deep Audio-Visual Embedding Network
}
\DeclareAcronym{accmultdavenet}{
	short = AcstMultDAVEnet,
	long  = acoustic multilingual deep audio-visual embedding network,
	alt = Acoustic Multilingual Deep Audio-Visual Embedding Network
}
\DeclareAcronym{DNN}{
	short = DNN,
	long  = deep neural network
}
\DeclareAcronym{ASR}{
	short = ASR,
	long  = automatic speech recognition
}
\DeclareAcronym{AWE}{
	short = AWE,
	long  = acoustic word embedding,
	alt = Acoustic Word Embedding
}
\DeclareAcronym{AGWE}{
	short = AGWE,
	long  = acoustically grounded word embedding,
	alt = Acoustically Grounded Word Embedding
}
\DeclareAcronym{ASE}{
	short = ASE,
	long  = acoustic span embedding,
	alt = Acoustic Span Embedding
}
\DeclareAcronym{QbE}{
	short = QbE,
	long  = query-by-example,
	alt  = Query-by-Example
}
\DeclareAcronym{STD}{
	short = STD,
	long  = spoken term detection
}
\DeclareAcronym{UTD}{
	short = UTD, 
	long = long short-term memory
}
\DeclareAcronym{SGD}{
	short = SGD, 
	long = stochastic gradient decent,
	alt = Stochastic Gradient Decent
}
\DeclareAcronym{bow}{
	short = BoW, 
	long = bag-of-words,
	alt = Bag-of-Words
}
\DeclareAcronym{mse}{
	short = MSE, 
	long = mean squared error,
	alt = Mean Squared Error
}
\DeclareAcronym{vpkl}{
	short = VPKL, 
	long = visually prompted keyword localisation,
	alt = Visually Prompted Keyword Localisation
}
\DeclareAcronym{vgs}{
	short = VGS,
	long  = visually grounded speech models,
	alt = Visually Grounded Speech Models
}


==> discussion.tex <==
\section{\leanne{Discussion}} %

We have shown that a visually grounded speech model exhibits the ME bias observed in young children~\cite{markman_childrens_1988,markman_categorization_1989}.
This bias has also been investigated in previous computational studies: both \citet{gulordava_deep_2020} and \citet{vong_cross-situational_2022} showed that neural networks taking images and written word labels as input exhibit a ME bias (in the latter case the results were, however, inconclusive).

\herman{[Did the paragraphs get messed up here?]}
\leanne{No, its exacly the same as what we handed in}
A major difference between our study and theirs is that we use real speech as input rather than written words.
Thanks to this, our visually grounded speech model better resembles the experimental setup with human participants and also makes the learning process more realistic.
Concretely, because the models in \citet{gulordava_deep_2020} and \citet{vong_cross-situational_2022} are trained on written words, which are discrete by design,
they need to learn a continuous embedding for each of the input classes.
However, this makes dealing with novel inputs difficult: if a model never sees a particular item at training time, its embeddings are never updated and remain randomly initialised. 
As a result, the ME test 
becomes a comparison of learned vs random embeddings instead of novel vs familiar.
To address this issue, \citet{gulordava_deep_2020} use novel examples in their contrastive loss during training, while \citet{vong_cross-situational_2022} perform one gradient update on novel classes before testing.
These strategies mean that, in both cases, the learner has actually seen the novel classes before testing.
Such adaptations are necessary in models taking in written input. 
In contrast, a visually grounded speech model, even when presented with an arbitrary input sequence, can place it in the representation space learned from the familiar classes during training.
Our results show that such a model exhibits the ME bias in a realistic setup where no adaptations are needed to deal with novel inputs.











==> implementation.tex <==
\section{Experimental setup}
\label{sec:implementation}

\subsection{Evaluation} 
\label{subsubsec:evaluations}

\begin{table*}[tb]
    \centering
    \small
    \caption{Summary of the evaluation setups in terms of the classes used for the query audio and the two given images. $F$ stands for familiar classes while $N$ stands for novel classes. The apostrophe indicates a different class, e.g.\ $F'$ will be a different familiar class than $F$. The last column gives the scores that we would see if a model has a perfect ME bias.}
    \label{tab:setup-summary}
    \begin{tabular}{lcccccc}
        \toprule
        & & Audio query & \multicolumn{2}{c}{Images' classes} & Perfect\\
        \cline{4-5}
        Evaluation & & class & Positive & Negative & accuracy if ME \\
        \midrule
        \Familiar & & $F$ & $F$ & $F'$ & 100\% \\
        \FamiliarWithNovel & & $F$ & $F$ & $N$ & 100\% \\
        \Me & & $N$ & $N$ & $F$ & 100\% \\
        \Novel & & $N$ & $N$ & $N'$ &  50\% \\
        \MeOther & & $N$ & $N'$ & $F$ & 100\% \\
        \bottomrule
    \end{tabular}
\end{table*}

Our main evaluation, is to test whether an ME bias naturally emerges in \model.
To evaluate this, we present the model with two image objects, one familiar and one novel.
The model is then prompted to identify which image belongs to a novel spoken word. 
To implement this, we sample 1000 episodes where each episode contains one spoken word query for each of the novel classes. 
For a novel query, we also sample two images, one containing the object for the novel class and the other containing a familiar object.
We refer to this as the \textit{ME} test.

To contextualise the ME results, we also perform four sanity checks. 
Two of these checks involve testing how accurately the model can discriminate familiar classes.
If the model does not know the familiar words, we cannot test whether the model has an ME bias.
The \textit{familiar vs novel} test uses the exact same episodes as the \textit{ME} test, but instead of using the novel spoken query, we use a spoken query for the familiar class.
The other test is the \textit{familiar} test which prompts the model to identify which of two familiar objects corresponds to a word query that matches one of the two classes.

The last two tests, stress tests the ME bias.
If indeed the model shows an ME bias, it should identify any novel object when prompted with a novel query.
Therefore, if we replace the familiar object in the \textit{ME} test with a novel object from a different novel class, the model should pick an image at random.
I.e.\ this score should be around 50\%.
And finally, we do the \textit{Mismatched ME} test which works exactly like the \textit{ME} test, but the novel query and novel object are from different novel classes. 
I.e.\ we adapt the \textit{ME} test by replacing the novel object with another one in the episode so that novel queries and objects are mismatched. 
This score should be %
similar to the ME score if the model indeed has an ME bias.
The different evaluation settings are summarised in Table~\ref{tab:setup-summary}.


\subsection{Models}
\label{sec:models}

Our goal is to establish whether \model\ uses an inherent ME bias to learn words. %
It is feasible to think that children have heard people speaking around them and visually interacted with the world around them~\cite{clark_how_2004}. 
As a result, we consider initialising the vision and audio branches of \model\ in an attempt to realistically replicate the environment in which children learn.
The two initialisation scenarios for the vision branch are random initialisation and using the pretrained convolutional AlexNet encoder where AlexNet is an object classification model.
\cite{soska_systems_2010} found that infants with more experience in interacting with visual objects, are better at making sense of novel objects.

For the audio branch, we also consider two initialisation scenarios: one using random initialisation and one where the acoustic network $f_{\textrm{acoustic}}$ is pretrained. 
This pretraining is done on Libri-Light~\cite{kahn_libri-light_2020} and the multilingual (English and Hindi) Places dataset~\cite{harwath_vision_2018}
using a self-supervised contrastive predictive coding task~\cite{van_niekerk_vector-quantized_2020}. 
With these initialisations, we end up with four possible \model\ variations as shown in column 2 and 3 in Table~\ref{tab:me}.

We test whether the visually grounded word learning model, \model\ shown in Fig.~\ref{fig:model}, has an inherent ME bias.
For the loss function in~\eqref{eq:loss}, we take $N_\textrm{pos}=5$ and $N_\textrm{neg}=11$.
All models are trained with Adam~\cite{kingma_adam_2015} for 100 epochs and early stopping with a validation task. 
During the validation task, the model is shown two images, both containing a familiar class.
The model is then prompted to identify which image corresponds to a word query (from one of these two classes). 
For this task, we use the spoken words and isolated object images from the development set.

